Smoothed Online Combinatorial Optimization Using Imperfect Predictions

Smoothed online combinatorial optimization considers a learner who repeatedly chooses a combinatorial decision to minimize an unknown changing cost function with a penalty on switching decisions in consecutive rounds. We study smoothed online combinatorial optimization problems when an imperfect predictive model is available, where the model can forecast the future cost functions with uncertainty. We show that using predictions to plan for a finite time horizon leads to regret dependent on the total predictive uncertainty and an additional switching cost. This observation suggests choosing a suitable planning window to balance between uncertainty and switching cost, which leads to an online algorithm with guarantees on the upper and lower bounds of the cumulative regret. Empirically, our algorithm shows a significant improvement in cumulative regret compared to other baselines in synthetic online distributed streaming problems.

==> abstract.tex <==
Smoothed online combinatorial optimization considers a learner who repeatedly chooses a combinatorial decision to minimize an unknown changing cost function with a penalty on switching decisions in consecutive rounds. We study smoothed online combinatorial optimization problems when an imperfect predictive model is available, where the model can forecast the future cost functions with uncertainty. We show that using predictions to plan for a finite time horizon leads to regret dependent on the total predictive uncertainty and an additional switching cost. This observation suggests choosing a suitable planning window to balance between uncertainty and switching cost, which leads to an online algorithm with guarantees on the upper and lower bounds of the cumulative regret. Empirically, our algorithm shows a significant improvement in cumulative regret compared to other baselines in synthetic online distributed streaming problems.


==> algorithm.tex <==
% \begin{align}
%     \max\nolimits_{P_0} & \quad \text{DesiredObjective}(P_0, P_{-0}) \\
%     \text{s.t.} & \quad P_i(D_{t,i}, P_{-i}, s_{t,i}) = D_{t,i} \quad ~\forall t \in [T], i \in [n]
% \end{align}

\begin{algorithm}[t]
\caption{Learning transition function in recurrent resource allocation}
\label{alg:learning-method}
\textbf{Input:} discount factor $0 < \gamma \leq 1$, switching cost $0 < \lambda$ \\
\textbf{Initialization:} predictive model $\model_\weight(\cdot)$ parameterized by neural network with weight $\weight$.
\tcp{Training resource allocation strategy}
\For{each training load balancing problem $f_1, f_2, \cdots, f_T$ with time horizon $T$} {
    \For{$t \in \{1, 2, \cdots T\}$}{
        Predict future traffic using data up to time $t-1$: $\{ \hat{f}_{s} \}_{s \geq t} = \model_\weight(\{ f_u \}_{u \leq t-1})$. \\
        Solve Equation~\ref{eqn:discrete-optimization-problem} using predicted traffic $\{ \hat{f}_{s} \}_{s \geq t}$ to get a new matching proposal $\matching_t$ at time $t$. \\
        Execute $\matching_t$ and observe the real traffic $f_t$ at time $t$. \\
        Define loss function to be either (i) two-stage loss: $\mathcal{L}_t = \norm{f_t - \hat{f}_t}$, or (ii) end-to-end decision-focused loss: $\mathcal{L}_t = \text{obj}(\matching_t, \matching_{t-1}, f_t)$ as defined in Equation~\ref{eqn:discrete-optimization-problem}.
    }
    Let $\mathcal{L} = \sum\nolimits_{t \in [T]} \mathcal{L}_t$. \\
    Compute $\frac{d \mathcal{L}}{d \weight}$ to run gradient descent and update model $\model_\weight$.
}
\textbf{Return:} resource allocation strategy $P_0$
\end{algorithm}

==> checklist.tex <==
\section*{Checklist}

\iffalse
%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%
\fi

\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{} 
  \item Did you describe the limitations of your work?
    \answerYes{Please refer to Section~\ref{sec:limitation-and-extension}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{Please refer to Appendix~\ref{sec:societal-impact}}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
   \answerYes{} 
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{} Please refer to Section~\ref{sec:proactive-planning}.
        \item Did you include complete proofs of all theoretical results?
    \answerYes{Please refer to Appendix.} 
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We will work on intellectual negotiations and make it available upon acceptance.} 
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Please refer to Section~\ref{sec:experiment}}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Please refer to Appendix~\ref{sec:computation-infrastructure}}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
   \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
  \answerNA{}
\end{enumerate}


\end{enumerate}

==> concentration.tex <==




\section{Concentration Bound of Randomized Rounding}
 
\begin{lemma}[Bernstein inequality]
Let $X_1, \cdots, X_n$ be independent zero-mean random variables. Suppose that $|X_i| \leq M$ almost surely, for all $i$. Then for all positive $t$,
\begin{align}
    \Pr\left[ \sum\limits_{i=1}^n X_i > t \right] \leq \exp \left( - \frac{t^2/2}{\sum\limits_{j=1}^n \E[X_j^2] + M t / 3} \right)
\end{align}
\end{lemma}



\begin{lemma}
Given $\parameter \in \R^k$, a binary assignment $\boldsymbol z \in \decisionset$, and the optimal solution $\decision^*$ of Equation~\ref{eqn:separated-optimization-problem-continuous}, let $\boldsymbol y_{ij}$ be a random variable with value $1$ with probability $\decision_{ij}$ and $0$ otherwise. If $C_{\min} \leq \parameter_i \leq C_{{\max}} ~\forall i$, then:
\begin{align}
    \Pr \left[ f(\boldsymbol y, \parameter) + \norm{\boldsymbol y - \boldsymbol z}_1 \geq c ( f(\decision^*, \parameter) + \norm{\decision - \boldsymbol z}_1) \right] \leq \delta
\end{align}
where $c = 2 \frac{C_{\max}}{C_{\min}} \sqrt{\log (m/\delta ) }$. \Zhao{Shouldn't we have some English/sentence, here?}
\end{lemma}
\begin{proof}
To prove the first inequality, recall that $f(\boldsymbol y, \parameter) = \norm{\boldsymbol y^\top \parameter}_\infty = \max_{j \in [m]} \sum\limits_{i=1}^k \boldsymbol y_{ij} \parameter_i$. So we just need to show the following inequality and apply union bound:
\begin{align}
    \Pr \Big[  \sum\limits_{i=1}^k \boldsymbol y_{ij} \parameter_i \geq c \sum\limits_{i=1}^k \decision_{ij} \parameter_i \Big] \leq \delta/m
\end{align}
\end{proof}


\begin{theorem}\label{thm:approximation-ratio-offline}
The solution obtained from applying continuous relaxation and randomized rounding to the following modified optimization problem in Equation~\ref{eqn:finite-optimization-problem-modified} is a $(1+\epsilon)S$-approximate solution to the optimization problem in Equation~\ref{eqn:finite-optimization-problem-polished}.
\end{theorem}
\begin{proof}


The last step is to ensure that the rounded solution of the continuous relaxation of Equation~\ref{eqn:finite-optimization-problem-polished} is not too far from its continuous solution, which is a lower bound of the binary solution.

\todo{
We can see that
\begin{align}
    \text{cost}(\text{OPT}_\text{conti.}) \leq \text{cost}(\decision_{\text{rounded}}) \leq (1 + \epsilon) \text{cost}(\text{OPT}_\text{conti.}) 
\end{align}
with high probability.

This part needs some work.
I need a condition on $\theta$ so that the randomized rounding outcome is an outcome of Poisson binomial distribution with small tail bound.
I don't have a quite thought on how to write this part for now.
}

This implies the performance of the rounded solution in Equation~\ref{eqn:finite-optimization-problem-modified} is upper bounded by $(1 + \epsilon)$ times of the continuous solution in Equation~\ref{eqn:finite-optimization-problem-modified}, which is again bounded by $(1 + \epsilon) S$ times of the continuous solution of Equation~\ref{eqn:finite-optimization-problem-polished} and thus also bounded by $(1 + \epsilon) S$ of the binary solution.
This completes the proof of approximation ratio of $(1 + \epsilon) S$ with high probability, where the high probability comes from the randomness of randomized rounding.
\end{proof}

==> idea.tex <==
\section{Some Thoughts}
\paragraph{Rounding of a continuous allocation}
Across both discrete and continuous settings, if we relax the variable $\mathcal{M}_t$ to a matrix with fractional values, the optimal sequential decision becomes a fractional resource assignment that is changing along with time $t$. It is not clear to me how to do rounding in order to keep the total variation small while maintaining the overall shape. This part sounds like an interesting research question to me.

\paragraph{Connection of reinforcement learning formulation and online/offline problems}
One important element in reinforcement learning formulation is how accurate we can learn the state transition function. Our state is composed of two parts: current traffic flow and previous action. If we have a transition function that can perfectly predict and recover the traffic flow, then the reinforcement learning problem falls into the offline case where the entire traffic flow is given in advance.
If the traffic flow is adversarial and thus cannot be easily predicted (I think the real case is either a Gaussian process or a Gaussian noise that are not fully predictable but also not adversarial), then the problem reduces to the online case.


\paragraph{Predictive accuracy of the transition function (incoming traffic) v.s. final performance}
One possible algorithm is to maintain a transition function to predict the incoming traffic. We can plan the future allocation scheme based on the transition function. When new data comes, we just update the transition function, make prediction on the future incoming traffic, and solve the offline problem based on the prediction in the next $T$ time steps. The performance of this algorithm will highly depend on the predictive accuracy of the transition function, and it is interesting to understand how the accuracy and the performance correlate.


\section{Useful Links}
\href{https://pipeline.gf.corp.adobe.com/d/pipe-kafka-looking-glass-prod/kafka-looking-glass?orgId=1&from=now-7d&to=now&var-data_source=v2-CORTEX-PROD&var-pipeline_cluster=NLD_A5&var-enm_cluster=ethos21prodnld2&var-kubernetes_namespace=ns-team-aep-pipeline-kafka-a5&var-cluster_name=pipeline-kafka&var-kafka_broker=All&var-kafka_topic=All&var-kafka_partition=All}{Adobe Pipeline Metric}

==> kafka.tex <==

\subsection{Kafka Scheduling Problem}
We assume there are in total $n$ partitions that we need to serve and $m$ brokers we can use to store data. Each partition $i \in [n]$ comes with a continuous traffic flow $f_i: \N  \longrightarrow \R_{\geq 0}$ (or multiple if there are multiple objectives). For each time step $t$, we use $f_t \in \R^n$ to denote the traffic vector. We use $f_{t,i}$ to denote the $i$-th coordinate of traffic vector, which is the traffic of $i$-th partition at time $t$.

Our goal is to construct a dynamic bipartite matching scheme $\matching$ to match partitions and brokers. We use a binary matrix $\matching_t \in \{0,1\}^{n \times m}$ to represent the matching assignment between $n$ partitions and $m$ brokers at time $t$. There are some linear constraints put on the matching assignment $\matching_t$, e.g., the number of partitions assigned to a single broker cannot exceed $4000$, and $\matching_t \mathbf{1}_m = \mathbf{1}_n$ to ensure that each partition is served by exactly one broker at a time, etc.

The load objective at time $t$ can be written as a function $g(\matching_t, f_t)$, e.g, we can define $g$ to be maximum of all the load $g(\matching_t^\top f_t) = \| \matching_t^\top f_t \|_{\infty}$ or define $g$ to be the variance of the load $\textbf{var}[\matching_t^\top f_t] = \| \matching_t^\top f_t - \E[\matching_t^\top f_t] \|_2^2$ which we want to minimize. Moreover, there is an additional switching cost incurred if the current bipartite matching $\matching_t$ is different from the last one $\matching_{t-1}$. The cost is denoted by $\lambda \norm{\matching_t - \matching_{t-1}}$ with a positive constant $\lambda$, where in this case we use the Hamming distance between two matchings as the norm function $\norm{\cdot}$. In this paper, we assume that there is a discount factor $0 < \gamma \leq 1$ for the future reward. Therefore, given traffic flow $f$ and matching scheme $\matching$, we can write down the cumulative objective by:
\begin{align}\label{eqn:objective}
    \sum_{t = 1}^T \gamma^t \cdot \text{obj}(\matching_t, \matching_{t-1}, f_t) \coloneqq \sum_{t = 1}^T \gamma^t \cdot \left( g(\matching_t, f_t) + \lambda \norm{\matching_{t} - \matching_{t-1}} \right)
\end{align}
%\Zhao{What is $\matching_0$? Is that all zero matrix or something else e.g. same as ${\cal M}_1$?} \Kai{We can have any arbitrary given initial point $\matching_0$. For example, it is probably just how the Kafka cluster is initially configured.} \Zhao{This makes sense.:)}

Our goal is to reduce such cumulative cost in the online setting, meaning that we do not have full access to the traffic flow $f$ but only have access up to time $t$ to make the decision $\matching_t$ online.

\subsection*{Challenges}
\begin{enumerate}
    \item Uncertain incoming traffic
    \item Future effect of chosen matching assignment and infinite time horizon
\end{enumerate}

==> learning.tex <==
\section{Learning Time Series with Changing Spectrum}

\begin{definition}[Sparse Deterministic Signal]
We assume that the traffic $f_t$ (for simplicify, let's just consider one dimensional traffic $f_t \in \R$) is the realization of a signal at time $t$ with sparse spectrum (Fourier transform). %\Zhao{In general, when we write equation, we don't use ``nolimits''. We probably do that if need to put more content in first 9 or 10 pages due to conference submission requirement.}
\begin{align}
    f_t = \sum_{j=1}^k a_j e^{2\pi i \theta_j t} + n(t)
\end{align}
for some $a_1, \cdots, a_k \in \C$, frequencies $\theta_1, \cdots, \theta_k \in \R$, and a Gaussian noise function $n(t)$.
\end{definition}

The goal is to recover the unknown parameters $a_i, \theta_i$ in as fewer samples as possible.



\begin{definition}[Sparse Signal with Noisy Amplitude]
We assume that the traffic $f_t$ (for simplicify, let's just consider one dimensional traffic $f_t \in \R$) is the realization of a signal at time $t$ with sparse spectrum (Fourier transform).
\begin{align}
    f_t = \sum_{j=1}^k a_j(t) e^{2\pi i \theta_j t} + n(t)
\end{align}
where $a_j(t) = b_j + n_j(t) \in \C$ are noisy realization of the amplitude at time $t$. $n(t), n_j(t)$ denote independent Gaussian noise functions.
\end{definition}
The problem becomes how to recover amplitude $a$ with as fewer samples as possible.



==> legacy.tex <==

composed of a resource manager who decides how to assign limited resources (budget), and a set of $n$ independently operating applications who maintain predictive models to predict the future demand and report back to the resource manager to get resources assigned.

The major challenge in this resource allocation problem is the uncertainty of the future demand in different distributed applications.
When the demand is given, we can feed all the demand information back to the resource management system. The resource management system solves an optimization problem to maximize the resource utilization and decide whether to shut down or bring up API service or Kafka clusters in certain Pipeline applications.
%When the future demand is low, resources are under utilized and can be shut down to save cost; when the future demand is high, resources have to be brought up to serve the incoming customer request.
However, the future demand information unfortunately is not known in advance. Very often a surge of demand suddenly appears in some applications and requires a great number of computing resources immediately.
To compensate such missing information, we can use the historical data to predict the future demand of each individual application.
The resource management system can gather these predictions to determine what action to take to handle the incoming demand and save cost.
We can see that prediction and allocation are two crucial components in this resource allocation process with uncertainty, where the whole process is depicted in Figure~\ref{fig:prediction} and Figure~\ref{fig:allocation}.

Additionally, these processes continue repeatedly, meaning that each individual application has to repeatedly predict the future demand and report back to the resource management system, and the resource management system has to make decision based on the predictions made by individual applications.
This is why we formulate the problem as a sequential resource allocation problem with future demand uncertainty.

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.8\textwidth}
         \centering
         \includegraphics[width=\textwidth]{flowcharts/prediction.pdf}
         \caption{Each individual application is facing an unknown future demand and maintains a time series predictive model to predict the future resource demand, e.g., API calls or computing demands. The resource management system has a certain budget to invoke computing clusters.}
         \label{fig:prediction}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.8\textwidth}
         \centering
         \includegraphics[width=\textwidth]{flowcharts/allocation.pdf}
         \caption{The resource manager receives all the predicted future demand from the individual applications and decides how to allocate resources (or reserve resources) to handle the incoming demands and optimize the resource utilization.}
         \label{fig:allocation}
     \end{subfigure}
    \caption{The illustration of the resource allocation problem composed of a predictive stage and an allocation stage. The whole process repeats in the next time step.}
    \label{fig:flowchart}
\end{figure}


\subsection{Time Series Prediction}
To predict the incoming future computing resource demand, we aim to use the historical API calls, customer counts, message usage, etc., to predict the future corresponding metrics and the required resources for each individual Pipeline application (region). This predictive problem is a time series prediction problem and is well-studied in many finance and weather forecasting problems. Given the uncertain nature of the incoming demand, the predictive model can not be perfect. Thus how to handle uncertainty in the later resource allocation part is another important role in our problem.

\subsection{Sequential Resource Allocation}
We assume there is resource management system that is responsible to decide how to allocate resources in order to align with the fixed budget constraint (or to maximize a common objective, e.g., to save cost) while simultaneously satisfying all the incoming demand. The resource management system collects the demand predictions made from all applications to decide how to shut down resources that are less likely to be used, and bring up resources in applications that are likely to be required.

If the predictions are perfect, the resource management system is facing a sequential decision problem where optimization or reinforcement learning approaches can be easily applied. We can adopt an optimization or a reinforcement learning algorithm to allocate resources to satisfy all the demands while minimizing the total cost. However, since the predictions are not perfect, the resource management system has to work with the uncertain predictions made by individual applications to achieve the best performance. To handle the uncertainty and potentially incorrect prediction, the resource management system can offer feedback to application to revise the predictive models based on the performance of the current predictions and the allocation rule. Simultaneously, the resource management system also needs to revise the allocation rule to handle the uncertainty in the prediction of future demand. 


\section{Project Goal}
Our goal is to build and train time series predictive models in all individual Pipeline applications, and learn an allocation rule to gather information and allocate resources under uncertainty.
We expect to build an end-to-end training process to have both prediction and the allocation components work together to improve the final performance of the whole sequential resource allocation system.




\subsubsection{Two-stage (TS) Learning Approach}
We can learn a time series predictive model $\model_\weight$ by updating the model weight based on the new observed traffic flow by comparing the prediction $\hat{f}_t$ and the observation $f_t$ to get a mismatch loss $\mathcal{L}_{\text{TS}}(f_t, \hat{f}_t) \coloneqq \| f_t - \hat{f}_t \|$. We can simply compute the gradient of $\mathcal{L}(f_t, \hat{f}_t)$ with respect to the model weight $\weight$ to run gradient descent to update the model.
The purpose of this learning approach is to find a predictive model that can minimize the predictive loss as much as possible.

However, our main goal is to optimize the objective that we really care, i.e., load balancing objective defined in Eq.~\eqref{eqn:objective}. Although predictive loss and the load balancing objective are correlated, they are not completely identical.

\subsubsection{Decision-focused (DF) Recurrent Optimization}
The discrepancy between predictive loss and the load balancing objective is the main motivation of end-to-end training. Instead of relying on minimizing predictive loss $\mathcal{L}_{\text{TS}}(f_t, \hat{f}_t) \coloneqq \| f_t - \hat{f}_t \|$, running gradient descent on the load balancing objective $\mathcal{L}_{\text{DF}}(f_t, \hat{f}_t) \coloneqq \text{obj}(\matching_t, \matching_{t-1}, f_t)$ can directly optimize the correct objective.

In order to compute the derivative of the load balancing objective with respect to the model parameter $\weight$, we apply chain rule to get:
\begin{align}
    \frac{\d ~\text{obj}(\matching_t, \matching_{t-1}, f_t)}{\d \weight} & = \frac{\d ~\text{obj}}{\d \matching_t} \frac{\d \matching_t}{\d \weight} + \frac{\d ~\text{obj}}{\d \matching_{t-1}} \frac{\d \matching_{t-1}}{\d \weight} \label{eqn:end-to-end-chain-rule} \\
    & = \frac{\d ~\text{obj}}{\d \matching_t} \left( \frac{\d \matching_t}{\d \hat{f}_{t}} \frac{\d \hat{f}_{t}}{\d \weight} + \frac{\d \matching_t}{\d \matching_{t-1}} \frac{\d \matching_{t-1}}{\d \weight} \right) + \frac{\d ~\text{obj}}{\d \matching_{t-1}} \frac{\d \matching_{t-1}}{\d \weight} \label{eqn:end-to-end-chain-rule-2} \\
    & = \frac{\d ~\text{obj}}{\d \matching_t} \frac{\d \matching_t}{\d \hat{f}_{t}} \frac{\d \hat{f}_{t}}{\d \weight} + \left( \frac{\d ~\text{obj}}{\d \matching_t} \frac{\d \matching_t}{\d \matching_{t-1}} + \frac{\d ~\text{obj}}{\d \matching_{t-1}} \right) \frac{\d \matching_{t-1}}{\d \weight} \label{eqn:end-to-end-chain-rule-3}
\end{align}

Since $\matching_t$ is the optimal solution to optimization problem in Eq.~\eqref{eqn:discrete-optimization-problem} with input variable $\hat{f}_t$ and $\matching_{t-1}$, we can apply the technique in differentiable optimization~\cite{amos2017optnet,agrawal2019differentiable} to compute the derivative of the optimal matching $\matching_t$ with respect to $\hat{f}_t$ and $\matching_{t-1}$, which we apply chain rule to Eq.~\eqref{eqn:end-to-end-chain-rule} to get Eq.~\eqref{eqn:end-to-end-chain-rule-2} backpropagate through $\hat{f}_{t}$ and $\matching_{t-1}$. 

However, since $\matching_{t-1}$ is also an optimal proposal at time $t-1$ and is a function of the previous prediction and proposal, we have to further expand the chain rule to get the correct derivative.
If we expand everything and compute all of them separately, this derivative computation can be very inefficient.
To save such computation cost, we notice that we can combine the parts with $\frac{\d \matching_{t-1}}{\d \weight}$ involved into one single term in Eq.~\eqref{eqn:end-to-end-chain-rule-3}.
This can largely save the computation cost of derivative from $O(T^2)$ to $O(T)$.

\begin{remark}
Since the variable $\matching_t$ needs to be binary so we need to apply randomized rounding to get from the continuous solution to binary. But since randomized rounding is not differentiable, we might need to relax all the $\matching_t$ to continuous variables during the learning phrase, and use randomized rounding only when we need to get a solution. This will become an approximate version of the end-to-end learning using differentiable optimization in sequential optimization setting, which is also something new and worth trying.
\end{remark}


%The main focus of this paper is to improve the efficiency of the backpropagation process.


The algorithm for these two methods is described in Algorithm~\ref{alg:learning-method}.

\input{algorithm}

==> lower.tex <==
\section{Lower Bound on The Cumulative Regret}
In the previous section, we show that our dynamic planning algorithm can achieve specific cumulative regret when the error rate satisfies certain structure, providing an upper bound on the cumulative regret that can be achieved.
In this section, we show that no randomized algorithm can achieve a cumulative regret lower than a certain order, which suggests a lower bound on the cumulative regret.


\begin{theorem}[Lower Bound]
Given uncertainty rate $\epsilon^{(t)}_{s} = \Theta(\frac{1}{t^b})$, there is no randomized algorithm that can guarantee cumulative regret of order $O(T^{1-b})$ when $b < 1$. When $b = 1$, there is no randomized algorithm that can guarantee cumulative regret $O(\log T)$
\end{theorem}
\begin{proof}
\todo{TODO}
Consider $n = 1$ and the traffic flow $f$ is a random process where $f_{t+1}$ is defined recursively based on $f_t$ as follows:
\begin{align*}
f_{t+1} = 
    \begin{cases}
      f_{t} + \epsilon_{t,1} \text{ with prob. } \frac{1}{2} \\
      f_{t} - \epsilon_{t,1} \text{ with prob. } \frac{1}{2}
    \end{cases}.
\end{align*}
\end{proof}

% \begin{theorem}
% The regret of Algorithm~\ref{alg:infinite-proactive-planning-full} is no worse the regret of  Algorithm~\ref{alg:infinite-proactive-planning} with high probability.
% \end{theorem}
% \begin{proof}

% \end{proof}

% \begin{corollary}
% Algorithm~\ref{alg:infinite-proactive-planning-full} is also no-regret if the confidence bound is asymptotically decreasing to $0$ with a polynomial with order $b > 0$.
% \end{corollary}



% \subsection{Solving Optimization Problem}
% Given traffic $f$ or the predicted traffic, solving the offline optimization in Eq.~\eqref{eqn:finite-optimization-problem} is still very challenging.
% If the decision variable is discrete, this problem becomes a high-dimensional combinatorial optimization problem with increasing time horizon.
% In particular, our algorithm requires that the horizon to be increasing to match to the potentially incurred switching cost.
% This makes solving the optimization problem even challenging and expensive.

% Previous works have shown that reinforcement learning algorithm can be used to solve hard combinatorial optimization problem like 3-SAT or Hamiltonian path problems.
% This motivates us to apply reinforcement learning algorithm to mitigate the challenge of solving high-dimensional problem.


\section{Combinatorial Optimization and Polynomial-time Approximation Scheme}
In the Kafka application, the feasible region is defined by $\decisionset = \{0,1\}^{k \times m}$, a binary allocation between $k$ partitions to $m$ brokers.
The parameter $\parameter_t \in \parameterset \subseteq \R^k$ is a $k$-dimensional vector where each entry $i$ denotes the traffic of partition $i$ at time $t$.
We use makespan, the maximal broker traffic across all brokers, as our objective function, i.e., $f(\decision, \parameter) = \max\limits_{j \in [m]} \sum\limits_{i \in [k]} \parameter_i x_{ij}$, or equivalently $f(\decision, \parameter) = \max(\parameter^\top \decision)$.
Given optimization window $S$ and all the predictions within the window $\theta_i$ for all $i \in [S]$, we can write the optimization problem as:
\begin{align}
    \min\limits_{\decision_t \in \decisionset \forall t \in [S]} & \quad \sum\limits_{t \in 1}^S f(\decision_t, \parameter_t) + d(\decision_t, \decision_{t-1}) \\
    \text{s.t. } & \quad x_t \boldsymbol1_m = \boldsymbol1_k
\end{align}

Or 
\begin{align}
    \min\limits_{\decision_t \in \decisionset \forall t \in [S]} & \quad \sum\limits_{t \in 1}^S \| \decision_t^\top \parameter_t \|_{\infty} + B |\decision_t - \decision_{t-1}| \\
    \text{s.t. } & \quad x_t \boldsymbol1_m = \boldsymbol1_k
\end{align}


\begin{align}
    \min\limits_{\decision_t \in \decisionset \forall t \in [S]} & \quad \sum\limits_{t \in 1}^S \| \decision_t^\top \parameter_t \|_{\infty} + 2 B |\decision_t - \decision_{0}| \\
    \text{s.t. } & \quad x_t \boldsymbol1_m = \boldsymbol1_k
\end{align}

% Well actually I can't even bound the integrality gap when $S=1$. The integrality gap might depend on $B$ as well and the discrepency of $x$. If $B$ is $0$, this problem is a bin packing problem. So if we have a large package $L$ and several small package with size $1$, the best we can do is to assign $L$ to one bin and all the others equally to the rest of $m-1$ bins, which yields makespan $L$. On the other hand, the best a fractional solution can do is $\frac{L+k-1}{m}$.

==> offline.tex <==

\section{Offline and Online Problems with Finite Time Horizon}
\subsection{Offline Problem}
Our first attempt is to solve the offline problem up to time $T$ with access to the entire future traffic vector $f$ to find the optimal dynamic matching assignment $\matching$.

\begin{definition}[Discrete]\label{def:discrete-optimization-problem}
Given a matrix ${\cal M}_{0} \in \{0,1\}^{n \times m}$, a collection of vectors $f_1, \cdots, f_T \in \R^n$ and a constraint vector $h \in \R^m$. Let $g$ denote a fixed function. Let $\lambda$ denote regularization parameter. 
The goal is to solve the following minimization problem with a future discount factor $0 < \gamma \leq 1$:
\begin{align}\label{eqn:discrete-optimization-problem}
    \min_{\matching \in \R^{n \times m \times T}} & \quad \sum_{t \in [T]} \gamma^t \left( g(\matching_t, f_t ) + \lambda \cdot \norm{\matching_{t} - \matching_{t-1}} \right) \\
    \mathrm{s.t.} & ~  \sum_{j \in [m]} M_{i,j,t} = 1 , & ~ \forall i \in [n], \forall t \in [T] ~\mathrm{(unique~assign)} \nonumber \\
    & ~ \sum_{i \in [n]} M_{i,j,t} \leq h_j, &  ~ \forall j \in [m], \forall t \in [T] ~\mathrm{(max~number~of~partitions)} \nonumber \\
    & ~ \matching_{t,i,j} \in \{0,1\} , & ~ \forall i \in [n], j \in [m], t \in [T] ~\mathrm{(discrete)} \nonumber
\end{align}
For any time $t \in [T]$, the above three constraints are ensuring the following properties:
\begin{itemize}
    \item each partition $i$ is severed by exactly one broker (e.g. broker $j$) at any time step $t$
    \item the number of partitions assigned to each broker $j$ is upper bounded by $h_j$.
    \item the assignment can not be fractional.
\end{itemize}
\end{definition}


\subsubsection{NP-hardness}
A special case of this problem is when $T = 1$ and there is no switching cost, i.e., $\lambda = 0$.
When $g$ is chosen to be the maximum over all the traffic across brokers, the problem reduces to the decision version of the bin packing problem: deciding whether $n$ items with given volume can be fit into $m$ bins each with certain size $K$.
\proof[Proof sketch]{
Supposing the offline optimization problem can be solved in polynomial time, we can feed the bin packing problem instance into the offline load balancing problem. If the load balancing problem gives an optimal objective less than $K$, then the answer is yes and otherwise no, which solves the decision version of the bin packing problem.
Since the decision version of the bin packing problem is NP-hard, this implies that the load balancing problem is at least NP-hard.
}

\subsubsection{Continuous Relaxation}\label{sec:continuous-relaxation}
One immediate step is to check how relaxation works to resolve the discreteness and how much approximation ratio we get there.
The problem becomes:
\begin{align}\label{eqn:discrete-optimization-problem-continuous-relaxation}
    \min\limits_{\matching \in \R^{n \times m \times T}} & \quad \sum\nolimits_{t \in [T]} g(\matching_t, f_t) + \lambda \norm{\matching_{t} - \matching_{t-1}} \\
    \mathrm{s.t.} & ~  \sum_{j \in [m]} M_{i,j,t} = 1 , & ~ \forall i \in [n], \forall t \in [T] ~\mathrm{(unique~broker)} \nonumber \\
    & ~ \sum_{i \in [n]} M_{i,j,t} \leq h_j, &  ~ \forall j \in [m], \forall t \in [T] ~\mathrm{(max~number~of~partitions)} \nonumber \\
    & ~ \matching_{t,i,j} \in [0,1] , & ~ \forall i \in [n], j \in [m], t \in [T] ~(\mathrm{bounded}) \nonumber
\end{align}

If function $g$ is convex in $\matching_t$, then the relaxed offline optimization problem is a convex optimization problem which can be solved efficiently.
In particular, both maximum over linear functions and variance over traffic flow that are commonly used in load balancing are both convex.

\paragraph{Research question} approximation ratio in the offline setting? Randomized rounding?

\subsection{Learning to Perform Greedy Algorithm on Combinatorial Problems}
The above discrete optimization problem is hard to solve precisely and the continuous relaxation can lose the optimality up to the approximation ratio.
Therefore, rather than predicting each individual traffic at different time step and optimizing accordingly using Eq.~\eqref{eqn:discrete-optimization-problem}, a more efficient way to solve the problem is to directly learn to run greedy algorithm.
We can maintain a value function $V$ to evaluate the future value of each partition broker assignment under historical traffic trend and last matching proposal.
The advantage of such greedy method is the efficiency of the optimization algorithm.
Since the optimization algorithm has to be run for every individual time step in a short time period, the algorithm needs to be efficient.
On the other hand, the disadvantage of the greedy method is that we are not sure whether the chosen valuation function can sufficiently represent the future value of each individual matching assignment.


\section{Online Problem}
\Kai{I feel that there are some impossibility results in the fully adversarial online version. Maybe we can construct some examples with large competitive ratio under different Lipschitz conditions.

The structure of the paper in my mind: offline version (binary: NP-hard, continuous: convex with approximation ratio), online version (impossibility result), RL version (proposed learning method).
} \Zhao{Sounds very promising plan.}

We would like to have an online dynamic matching scheme $\matching$ where $\matching_t$ is a function of historical data $f_1, f_2, \cdots, f_{t-1} \in \R^{n}_{\geq 0}$ and the previous matching proposal $\matching_{t-1}$.

%\Zhao{We probably can make the following mild assumption. This sounds very interesting.}

The following two assumptions are inspired by \cite{cls19}.
\begin{assumption}[slowly change per iteration]\label{assumption:slow-change-per-iteration}
We assume that
\begin{align*}
    \| f_t - f_{t-1} \| \leq \epsilon, \forall t \in [T]
\end{align*}
\end{assumption}
The following assumption is weaker than the above one.

\begin{assumption}[slowly change over the all the iterations]\label{assumption:slow-change-entire-itartions}
We assume that
\begin{align*}
    \sum_{t=1}^T \| f_t - f_{t-1} \| \leq \epsilon
\end{align*}
\end{assumption}

\begin{assumption}[Bounded traffic flow]
We assume that the traffic vector is upper bounded by $U$:
\begin{align}
    0 \leq f_{t,i} \leq U ~\forall t, i
\end{align}

\end{assumption}

% \paragraph{Property of traffic vector} In our setting, the incoming traffic vector is smooth and Lipchitz. We also assume there is a periodic pattern of the traffic vector. It is not clear to me how to formally define such assumption yet.


\subsection{Passive Planning: Optimization Over Previous Traffic}
Given that the traffic is slowly changing, a naive algorithm is to optimize against the previous traffic flow to determine what new matching scheme to adopt.
The main motivation of using the previous traffic flow is because the traffic flow with high probability will not change much.
The algorithm is shown in Algorithm~\ref{alg:naive-online-algorithm}.

\begin{algorithm}[h]
\caption{Naive Online Algorithm}
\label{alg:naive-online-algorithm}
\textbf{Input:} $n,m$, initial matching $\matching_0$ \\
    \For{$t \in \{1, 2, \cdots T\}$}{
        Find $\matching_t$ to minimize $ \text{obj}(\matching_t, \matching_{t-1}, f_{t-1})$ \\
        Execute $\matching_t$ and observe the real traffic $f_t$ at time $t$. \\
        Receive objective $ \text{obj}(\matching_t, \matching_{t-1}, f_{t})$
    }
\textbf{Return:} resource allocation strategy $P_0$
\end{algorithm}

This naive algorithm can lead to constantly worse performance compared to the optimal solution to the offline problem when the incoming traffic in the online problem is chosen adversarially.
\begin{theorem}
Suppose $g(\matching, f) = \max\limits_{j \in [m]} \{\matching^\top f\}_j$. When there is no switching cost $\lambda = 0$, the naive algorithm can be $O(\epsilon TL)$ close to the offline optimal solution at time $T$, where $L$ is the Lipschitzness of $g$ in terms of $f$.
\end{theorem}
\begin{proof}
At time $t$, since we are optimizing over the previous traffic $f_{t-1}$, the current traffic $f_t$ can be slightly different from the previous traffic $f_{t-1}$ but at most $\norm{f_t - f_{t-1}} \leq \epsilon$.
We can write the proposed matching and the optimal matching by:
\begin{align}
    \matching_t &= \arg\min_{\matching_t} \text{obj}(\matching_t, \matching_{t-1}, f_{t-1}) = g(\matching_t, f_{t-1}) + \lambda \norm{\matching_t - \matching_{t-1}} \label{eqn:no-switching-cost-optimality-1} \\
    \matching_t^* &= \arg\min_{\matching_t} \text{obj}(\matching_t, \matching_{t-1}, f_{t}) = g(\matching_t, f_{t}) + \lambda \norm{\matching_t - \matching_{t-1}} \label{eqn:no-switching-cost-optimality-2}
\end{align}

By Equation~\ref{eqn:no-switching-cost-optimality-1}, we have:
\begin{align}
    \text{obj}(\matching_t, \matching_{t-1}, f_{t-1}) \leq  \text{obj}(\matching^*_t, \matching_{t-1}, f_{t-1}) \nonumber \\
    \text{obj}(\matching_t, \matching_{t-1}, f_{t-1}) - \text{obj}(\matching^*_t, \matching_{t-1}, f_{t-1}) \leq 0 \label{eqn:no-switching-cost-telescoping-1}
\end{align}

By Lipchitzness of function $g$, we have:
\begin{align}
    \text{obj}(\matching_t, \matching_{t-1}, f_t) - \text{obj}(\matching_t, \matching_{t-1}, f_{t-1}) = & g(\matching_t, f_t) - g(\matching_{t}, f_{t-1}) \nonumber \\
    = & \frac{\partial g}{\partial f} \norm{f_t - f_{t-1}} \leq L \epsilon \label{eqn:no-switching-cost-telescoping-2} \\
    \text{obj}(\matching_t^*, \matching_{t-1}, f_{t-1}) - \text{obj}(\matching_t^*, \matching_{t-1}, f_{t}) \leq & L \epsilon \label{eqn:no-switching-cost-telescoping-3}
\end{align}

Taking summation over Equation~\ref{eqn:no-switching-cost-telescoping-1}, ~\ref{eqn:no-switching-cost-telescoping-2}, and ~\ref{eqn:no-switching-cost-telescoping-3}, we get a telescoping sum:
\begin{align}
    \text{obj}(\matching_t, \matching_{t-1}, f_t) - \text{obj}(\matching_t^*, \matching_{t-1}, f_{t}) \leq 2 L\epsilon \nonumber
\end{align}
Due to the optimality of $\matching_t^*$ from Equation~\ref{eqn:no-switching-cost-optimality-2}, we also know that:
\begin{align}
    \text{obj}(\matching_t^*, \matching_{t-1}, f_{t}) \leq \text{obj}(\matching_t, \matching_{t-1}, f_{t}) \nonumber
\end{align}

Thus we conclude that
\begin{align}
    |\text{obj}(\matching_t, \matching_{t-1}, f_t) - \text{obj}(\matching_t^*, \matching_{t-1}, f_{t}) | \leq 2 L \epsilon \nonumber
\end{align}
This implies that every round can only incur at most $2L \epsilon = O(\epsilon L)$ regret. Across $T$ rounds, the regret is bounded by $O(\epsilon TL)$.
\end{proof}

Notice that the Lipschitz constant $L$ depends on the definition of the objective function $g$. In particular, we can write $L = \sup \norm{\frac{\partial g}{\partial f}}$. In the case where $g(\matching, f) = \max\limits_{j \in [m]} \{\matching^\top f\}_j$, the partial derivative is exactly the $M_j$ where $j = \arg\max_{j \in [m]} \{ \matching^\top f \}_j$. Thus we can bound the norm of the partial derivative by $L = \sup \norm{M_j} = \sqrt{n}$.
In the above case, the regret bound becomes $O(\sqrt{n} \epsilon)$.

\begin{theorem}
Suppose $g(\matching, f) = \max\limits_{j \in [m]} \{\matching^\top f\}_j$.
When there is a switching cost $\lambda > 0$ with arbitrary $\epsilon$, the naive algorithm can be $O(n \lambda T)$ worse than the offline optimal solution at time $T$.
In the discounted case, the naive algorithm can be $O(\frac{1}{1 - \gamma} n \lambda)$ worse than the offline optimal solution.
%If the initial matching proposal is optimal, the naive algorithm can be $\frac{\gamma^{\frac{\lambda}{\epsilon}}}{1 - \gamma} (n-1) \lambda$ worse than the optimal solution.
\end{theorem}
\begin{proof}
Consider an instance with $n$ partitions and $m=2$ brokers.
Suppose the initial traffic has $f_0 = [(n-1)(\lambda - \delta), (\lambda - \delta), (\lambda - \delta), \cdots, (\lambda - \delta)]^\top$ and the initial matching is to assign partitions $\{1,2,\cdots, n-1\}$ to the first broker and partition $n$ to the second broker with a maximal traffic $(2n-3) \lambda$. This initial matching assignment is $(n-2)\lambda$ worse than the optimal solution, where the optimal solution is to assign all the partitions with traffic $\lambda$ to one broker and the one with traffic $(n-1) \lambda$ to the other broker with a maximal traffic $(n-1) \lambda$.
However, there is also no incentive to switch to any other matching assignment due to the associated switching cost $\lambda$.
Thus the naive algorithm incurs a regret $(n-2)\lambda$ at each round and never changes the matching assignment which results in a cumulative regret $O(n\lambda T)$. In the discounted case, this results in $O(\frac{1}{1-\gamma} n \lambda)$.
\end{proof}


\begin{remark}
Ignoring the switching cost to find the optimal matching assignment does not resolve the issue because ignoring the switching cost itself can incur $O(n \lambda)$ additional cost at each round.
\end{remark}

